[Re] Double Sampling Randomized Smoothing

This paper is a contribution to the reproducibility challenge in the field of machine learning, specifically addressing the issue of certifying the robustness of neural networks (NNs) against adversarial perturbations. The proposed Double Sampling Randomized Smoothing (DSRS) framework overcomes the limitations of existing methods by using an additional smoothing distribution to improve the robustness certification. The paper provides a clear manifestation of DSRS for a generalized family of Gaussian smoothing and a computationally efficient method for implementation. The experiments on MNIST and CIFAR-10 demonstrate the effectiveness of DSRS, consistently certifying larger robust radii compared to other methods. Also various ablations studies are conducted to further analyze the hyperparameters and effect of adversarial training methods on the certified radius by the proposed framework.

==> graphs/graph_1.tex <==
\pgfplotsset{every x tick label/.append style={font=\scriptsize}}
\resizebox{6cm}{!}{%
\begin{tikzpicture}
    \begin{axis}[
        title={The Variation of ACR and N },
        xlabel={Sampling Number (N) for P },
        ylabel={Average Certified Radius (ACR)},
        xmin=0, xmax=60000,
        ymin=0, ymax=0.7,
        xtick={50, 100, 500, 2000, 8*1e3, 20*1e3, 50*1e3},
        ytick={0, 0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7},
        legend pos=south east,
        ymajorgrids=true,
        grid style=dashed,
        xmode=log,
        log ticks with fixed point,
        % for log axes, x filter operates on LOGS.
        % and log(x * 1000) = log(x) + log(1000):
        scaled x ticks=real:1e3
    ]

        \addplot[
            color=blue,
            mark=square,
            ]
            coordinates {
            (50,0.157)(100,0.227)(500,0.341)(2000,0.403)(8000,0.441)(20000,0.459)(50000,0.456)
            };
        \addlegendentry{Cifar10-half-Gaussian}
        \addplot[
            color=red,
            mark=square,
            ]
            coordinates {
            (50,0.193)(100,0.269)(500,0.404)(2000,0.486)(8000,0.548)(20000,0.582)(50000,0.611)
            };
        \addlegendentry{Cifar10-half-Consistency}

        \addplot[
            color=green,
            mark=square,
            ]
            coordinates {
            (50,0.206)(100,0.286)(500,0.429)(2000,0.515)(8000,0.580)(20000, 0.614)(50000,0.628)
            };
        \addlegendentry{Cifar10-half-Smoothmix}

    \end{axis}
\end{tikzpicture}%
}

==> graphs/graph_2.tex <==
\resizebox{6cm}{!}{%
\begin{tikzpicture}
    \begin{axis}[
        title={The Variation of ACR and K },
        xlabel={K (General-Gaussian) },
        ylabel={Average Certified Radius (ACR)},
        xmin=0, xmax=1600,
        ymin=0.5, ymax=0.7,
        xtick={0, 200,400,600,800,1000,1200,1400,1600},
        ytick={0.5,0.55, 0.6,0.65, 0.7},
        legend pos=south east,
        ymajorgrids=true,
        grid style=dashed,
    ]
        \addplot[
        % DSRS Radius
            color=blue,
            mark=square,
            ]
            coordinates {
            (0, 0.658)(200,0.654)(400,0.655)(600,0.655)(800,0.655)(1000,0.655)(1200,0.655)(1400,0.652)(1521,0.631)(1525,0.626)(1529,0.615)(1533,0.561)
            };
    \addlegendentry{Cifar10-half-Consistency-DSRS}
    \addplot[
    % Neyman Pearson Radius
            color=red,
            mark=square,
            ]
            coordinates {
            (0, 0.681)(200,0.677)(400,0.677)(600,0.678)(800,0.677)(1000,0.677)(1200, 0.676)(1400,0.674)(1521,0.646)(1525,0.636)(1529,0.616)(1533,0.554)
            };
    \addlegendentry{Cifar10-half-Consistency-N-P}
    \end{axis}
\end{tikzpicture}%
}

==> graphs/graph_3.tex <==
\resizebox{6cm}{!}{%
\begin{tikzpicture}
    \begin{axis}[
        title={The Variation of ACR and $ \sigma_P $ },
        xlabel={$ \sigma_P $ (General-Gaussian) },
        ylabel={Average Certified Radius (ACR)},
        xmin=0, xmax=1,
        ymin=0.1, ymax=0.75,
        xtick={0,0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
        ytick={0.1, 0.2, 0.3, 0.4, 0.5, 0.6, 0.7},
        legend pos=south east,
        ymajorgrids=true,
        grid style=dashed,
    ]
       \addplot[
            color=blue,
            mark=square,
            ]
            coordinates {
            (0.05, 0.135)(0.10, 0.238)(0.20, 0.396)(0.25, 0.358)
            (0.5,0.456)(1.0,0.473)
            };
        \addlegendentry{Cifar10-half-Gaussian}
        \addplot[
            color=red,
            mark=square,
            ]
            coordinates {
            (0.05, 0.133)(0.10, 0.236)(0.20, 0.388)(0.25, 0.452)
            (0.5,0.611)(1.0,0.651)
            };
        \addlegendentry{Cifar10-half-Consistency}

        \addplot[
            color=green,
            mark=square,
            ]
            coordinates {
            (0.05, 0.122)(0.10, 0.223)(0.20, 0.384)(0.25, 0.451)
            (0.5,0.628)(1.0,0.707)
            };
        \addlegendentry{Cifar10-half-Smoothmix}
    \end{axis}
\end{tikzpicture}%
}

==> graphs/graph_4.tex <==
\resizebox{6cm}{!}{%
\begin{tikzpicture}
    \begin{axis}[
        title={The Variation of ACR and $ \sigma_Q $ ($ \sigma_P = 0.5 $) },
        xlabel={$ \sigma_Q $},
        ylabel={Average Certified Radius (ACR)},
        xmin=0, xmax=1.0,
        ymin=0.3, ymax=0.7,
        xtick={0, 0.1, 0.2,0.3, 0.4, 0.5, 0.6, 0.7, 0.8, 0.9, 1.0},
        ytick={0.3,0.35, 0.4,0.45, 0.50,0.55, 0.6,0.65, 0.7},
        legend pos=south east,
        ymajorgrids=true,
        grid style=dashed,
    ]

        \addplot[
            color=blue,
            mark=square,
            ]
            coordinates {
            (0.1,0.447)(0.2,0.447)(0.3,0.461)(0.4,0.472)(0.5,0.447)(0.6,0.447)(0.7,0.447)(0.8,0.447)(0.9,0.447)
            };
        \addlegendentry{Cifar10-half-Gaussian}
        \addplot[
            color=red,
            mark=square,
            ]
            coordinates {
            (0.1,0.590)(0.2,0.590)(0.3,0.598)(0.4,0.609)(0.5,0.590)(0.6,0.590)(0.7,0.590)(0.8,0.590)(0.9,0.590)
            };
        \addlegendentry{Cifar10-half-Consistency}

        \addplot[
            color=green,
            mark=square,
            ]
            coordinates {
            (0.1,0.620)(0.2,0.620)(0.3,0.630)(0.4,0.642)(0.5,0.620)(0.6,0.620)(0.7,0.620)(0.8,0.620)(0.9,0.620)
            };
        \addlegendentry{Cifar10-half-Smoothmix}

    \end{axis}
\end{tikzpicture}%
}
